Solving the Weighted HOM-Problem With the Help of Unambiguity

The HOM-problem, which asks whether the image of a regular tree language under a tree homomorphism is again regular, is known to be decidable by [Godoy, Gim\'enez, Ramos, \`Alvarez: The HOM problem is decidable. STOC (2010)]. Research on the weighted version of this problem, however, is still in its infancy since it requires customized investigations. In this paper we address the weighted HOM-problem and strive to keep the underlying semiring as general as possible. In return, we restrict the input: We require the tree homomorphism h to be tetris-free, a condition weaker than injectivity, and for the given weighted tree automaton, we propose an ambiguity notion with respect to h. These assumptions suffice to ensure decidability of the thus restricted HOM-problem for all zero-sum free semirings by allowing us to reduce it to the (decidable) unweighted case.

==> eptcsdata.tex <==
\providecommand{\firstpage}{200}
\providecommand{\publicationstatus}{Zs. Gazdag, Sz. Iv\'an, G. Kov\'asznai (Eds.): 16th International\\Conference on Automata and Formal Languages (AFL 2023)\\
EPTCS 386, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.386.16}{10.4204/EPTCS.386.16}}

